Cross-platform validation and analysis environment for particle physics

A multi-platform validation and analysis framework for public Monte Carlo simulation for high-energy particle collisions is discussed. The front-end of this framework uses the Python programming language, while the back-end is written in Java, which provides a multi-platform environment that can be run from a web browser and can easily be deployed at the grid sites. The analysis package includes all major software tools used in high-energy physics, such as Lorentz vectors, jet algorithms, histogram packages, graphic canvases, and tools for providing data access. This multi-platform software suite, designed to minimize OS-specific maintenance and deployment time, is used for online validation of Monte Carlo event samples through a web interface.

==> Makefile <==
NOTENAME = jhepsim
TEX := latex

.PHONY: all clean

all:#default target makes everything
	$(TEX) $(NOTENAME).tex
	bibtex $(NOTENAME)
	$(TEX) $(NOTENAME).tex
	bibtex $(NOTENAME)
	bibtex $(NOTENAME)	
	$(TEX) $(NOTENAME).tex
	dvips $(NOTENAME)
	ps2pdf $(NOTENAME).ps  $(NOTENAME).pdf 
show:
	evince $(NOTENAME).pdf

clean:
	rm -rf $(NOTENAME).aux $(NOTENAME).log $(NOTENAME).out $(NOTENAME).bbl $(NOTENAME).blg \
	$(NOTENAME).dvi $(NOTENAME).ps \
	$(NOTENAME).toc $(NOTENAME).tof thumb*.* $(NOTENAME).pdf

